SkillScope: A Tool to Predict Fine-Grained Skills Needed to Solve Issues on GitHub

New contributors often struggle to find tasks that they can tackle when onboarding onto a new Open Source Software (OSS) project. One reason for this difficulty is that issue trackers lack explanations about the knowledge or skills needed to complete a given task successfully. These explanations can be complex and time-consuming to produce. Past research has partially addressed this problem by labeling issues with issue types, issue difficulty level, and issue skills. However, current approaches are limited to a small set of labels and lack in-depth details about their semantics, which may not sufficiently help contributors identify suitable issues. To surmount this limitation, this paper explores large language models (LLMs) and Random Forest (RF) to predict the multilevel skills required to solve the open issues. We introduce a novel tool, SkillScope, which retrieves current issues from Java projects hosted on GitHub and predicts the multilevel programming skills required to resolve these issues. In a case study, we demonstrate that SkillScope could predict 217 multilevel skills for tasks with 91% precision, 88% recall, and 89% F-measure on average. Practitioners can use this tool to better delegate or choose tasks to solve in OSS projects.

==> domains_subdomains.tex <==

Application & Integration & Plugin Management & User Customization & App Configuration & Version Control & Compatibility Checks \\
\hline
Application Performance Manager & Performance Monitoring & Resource Allocation & Error Detection & Load Balancing & Traffic Management & Diagnostic Tools \\
\hline
Big Data & Data Processing & Data Storage & Data Analysis & Real-Time Processing & Batch Processing & Data Visualization \\
\hline
Cloud & Resource Management & Virtualization & Scalability Solutions & Cloud Security & Data Migration & Service Configuration \\
\hline
Computer Graphics & Image Rendering & Animation & Modeling & Texture Mapping & Visual Effects & Graphics Optimization \\
\hline
Data Structure & Linear Structures & Tree Structures & Graph Structures & Data Sorting & Search Algorithms & Data Manipulation \\
\hline
Databases & Query Execution & Transaction Management & Schema Design & Database Security & Backup and Recovery & Database Optimization \\
\hline
Software Development and IT Operations & Continuous Integration & Continuous Deployment & Automated Testing & Configuration Management & Version Control & Monitoring and Logging \\
\hline
Error Handling & Exception Handling & Error Logging & Fault Tolerance & Debugging Tools & User Notification & Error Prevention \\
\hline
Event Handling & User Interactions & System Events & Event Logging & Event Driven Processing & Notifications & Asynchronous Processing \\
\hline
Geographic Information System & Mapping & Spatial Analysis & Data Collection & Geographic Visualization & Location Services & Environmental Modeling \\
\hline
Input-Output & Data Reading & Data Writing & Stream Management & Buffering Strategies & File Management & Network IO \\
\hline
Interpreter & Script Execution & Code Translation & Memory Management & Syntax Analysis & Optimization & Debugging \\
\hline
Internationalization & Localization & Language Support & Cultural Adaptation & Currency Conversion & Date/Time Formatting & Right-to-Left Layouts \\
\hline
Logic & Control Structures & Algorithm Implementation & Logic Optimization & Validation Checks & Rule Processing & Decision Making \\
\hline
Language & Syntax Features & Compiler/Interpreter Enhancements & Runtime Optimization & Standard Libraries & Language Extensions & Type Systems \\
\hline
Logging & Event Logging & System Monitoring & Performance Tracking & Error Logs & User Activity Logs & Audit Trails \\
\hline
Machine Learning & Training Models & Prediction & Data Preprocessing & Feature Extraction & Model Evaluation & Deployment \\
\hline
Microservices and Services & Service Discovery & Load Balancing & API Gateway & Service Communication & Fault Tolerance & Service Deployment \\
\hline
Multimedia & Media Playback & Media Editing & Encoding and Decoding & Streaming & Content Delivery & Media Storage \\
\hline
Multi-Thread & Concurrency Control & Synchronization & Thread Safety & Parallel Processing & Resource Sharing & Deadlock Resolution \\
\hline
Natural Language Processing & Text Analysis & Speech Recognition & Language Generation & Sentiment Analysis & Machine Translation & Chatbot Interfaces \\
\hline
Network & Protocol Implementation & Connection Management & Data Transmission & Network Security & Bandwidth Optimization & Network Monitoring \\
\hline
Operating System & Process Management & Memory Management & Device Drivers & File Systems & User Interface & System Security \\
\hline
Parser & Syntax Parsing & Error Recovery & Data Conversion & Optimization & Code Generation & Validation \\
\hline
Search & Indexing & Query Processing & Ranking & Optimization & Caching & Personalization \\
\hline
Security & Authentication & Authorization & Encryption & Intrusion Detection & Compliance & Data Integrity \\
\hline
Setup & Installation & Configuration & System Requirements & Update Management & Licensing & Environment Setup \\
\hline
User Interface & Layout Design & Interaction Design & Accessibility & Animation & Responsive Design & User Feedback \\
\hline
Utility & Data Conversion & System Tools & Automation Scripts & Performance Tools & Diagnostic Utilities & Backup Tools \\
\hline
Test & Unit Testing & Integration Testing & Performance Testing & Security Testing & Usability Testing & Regression Testing

==> llm_performance.tex <==
Average & Precision (1) & Recall (1) & F1 (1) \\ 
\hline %\hline
% Computer Graphics                                             & 0.27     & 0.78          & 0.03       & 0.00   & 0.26          & 0.97       & 0.41   \\
% Data Structure-Tree Structures                                & 0.30     & 0.91          & 0.09       & 0.02   & 0.25          & 0.97       & 0.40   \\
% Data Structure-Search Algorithms                              & 0.24     & 0.75          & 0.01       & 0.00   & 0.24          & 0.99       & 0.39   \\
% Data Structure-Data Manipulation                              & 0.33     & 0.65          & 0.23       & 0.12   & 0.22          & 0.64       & 0.33   \\
% Databases                                                     & 0.25     & 0.53          & 0.04       & 0.01   & 0.24          & 0.91       & 0.38   \\
% Software Development and IT Operations-Version Control        & 0.55     & 0.80          & 0.58       & 0.49   & 0.20          & 0.43       & 0.27   \\
% Software Development and IT Operations-Monitoring and Logging & 0.24     & 0.61          & 0.06       & 0.01   & 0.21          & 0.86       & 0.34   \\
% Error Handling                                                & 0.36     & 0.78          & 0.25       & 0.12   & 0.22          & 0.75       & 0.34   \\
% Logic                                                         & 0.30     & 0.60          & 0.18       & 0.08   & 0.22          & 0.65       & 0.33   \\
% Language-Standard Libraries                                   & 0.32     & 0.83          & 0.15       & 0.05   & 0.24          & 0.90       & 0.38   \\
% Parser                                                        & 0.27     & 0.78          & 0.08       & 0.01   & 0.23          & 0.93       & 0.37   \\
% User Interface-Layout Design                                  & 0.34     & 0.77          & 0.20       & 0.08   & 0.24          & 0.80       & 0.37   \\
% User Interface-Interaction Design                             & 0.53     & 0.90          & 0.47       & 0.32   & 0.26          & 0.79       & 0.39   \\
% User Interface-Accessibility                                  & 0.21     & 0.45          & 0.04       & 0.01   & 0.19          & 0.82       & 0.31   \\
% User Interface-User Feedback                                  & 0.44     & 0.73          & 0.38       & 0.26   & 0.25          & 0.59       & 0.35   \\
% \hline
Micro     & 0.76    & 0.21     & 0.36      \\
Macro               
& 0.73     & 0.19     & 0.30   \\      
\hline
Average & Precision (0) & Recall (0) & F1 (0) \\
Micro & 0.23     & 0.80     & 0.36 \\
Macro  & 0.23     & 0.80     & 0.36 \\



%Micro     & 0.33           & 0.76    & 0.21     & 0.36      & 0.23     & 0.80     & 0.36 \\
%Macro     & 0.33          
%& 0.73     & 0.19     & 0.30   & 0.23     & 0.80     & 0.36 \\   

==> notused.tex <==
\subsection{Parse Source Code}\label{sec:parse}
// TEAM CORE ENGINE - One subsection for parsing and building ASTs, Identifying APIs and functions context and domains
// We don't need to go into details like I run the g4f function x to execute y.

//Explain the way you explain in a high level to a technical customer

\subsection{Data Mining}\label{sec:mining}
// TEAM DATA MINING - One subsection for every topic: mining software repository, fusion, and cleaning
// Explain how you mined the project's data and describe the columns

// Explain the dataset

\subsection{Predictions}\label{sec:predictions}
//TEAM PREDICTIONs - one section for each ML algorithm - LLM/classic/BERT
// Explain the ML models

//Explain the feature selection

// Explain the tuning

\subsection{User Study}

// TEAM UI
// How can we test whether the UI improved the context for contributors?

// Summarize a possible user study to measure this

// ALL TEAMS
//Describe step by step each teamwork (engine, data mining, prediction)
\subsection{Data Analysis}\label{sec:dataanalysis}
//Explain the stat test (if any)
// ALL TEAMS
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

\author{\IEEEauthorblockN{1\textsuperscript{st} Benjamin C. Carter}
\IEEEauthorblockA{\textit{CET} \\
\textit{Grand Canyon University}\\
Phoenix, AZ \\
BCarter44@my.gcu.edu}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Dylan Johnson}
\IEEEauthorblockA{\textit{CET} \\
\textit{Grand Canyon University}\\
Phoenix, AZ \\
DJohnson457@my.gcu.edu}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Carlos A. Llanes Villegas}
\IEEEauthorblockA{\textit{CET} \\
\textit{Grand Canyon University}\\
Phoenix, AZ \\
carlos.llanes.villegas@gmail.com}
\and
\IEEEauthorblockN{4\textsuperscript{th}Adonijah O. Farner}
\IEEEauthorblockA{\textit{CET} \\
\textit{Grand Canyon University}\\
Phoenix, United States \\
adon.farner@gmail.com}
\and
\IEEEauthorblockN{5\textsuperscript{th} Hunter Jenkins}
\IEEEauthorblockA{\textit{CET} \\
\textit{Grand Canyon University}\\
Phoenix, USA \\
huntermjenkins@gmail.com}
\and
\IEEEauthorblockN{6\textsuperscript{th} Jack Utzerath}
\IEEEauthorblockA{\textit{CET} \\
\textit{Grand Canyon University}\\
Phoenix, USA \\
jackutz@live.com}
\and
\IEEEauthorblockN{7\textsuperscript{th} Jonathan Rivas Contreras}
\IEEEauthorblockA{\textit{CET} \\
\textit{Grand Canyon University}\\
Phoenix, USA \\
JRivas20@my.gcu.edu}
\and
\IEEEauthorblockN{8\textsuperscript{th} Jacob Penney}
\IEEEauthorblockA{\textit{SICCS} \\
\textit{Northern Arizona University}\\
Flagstaff, USA \\
jacob\_penney@nau.edu}
\and
\IEEEauthorblockN{9\textsuperscript{th} Fabio Santos}
\IEEEauthorblockA{\textit{CET} \\
\textit{Grand Canyon University}\\
Phoenix, USA \\
fabiomarcos.deabre@gcu.edu}
\and
\IEEEauthorblockN{10\textsuperscript{th} Igor Steinmacher}
\IEEEauthorblockA{\textit{SICCS} \\
\textit{Northern Arizona University}\\
Flagstaff, USA \\
igor.steinmacher@nau.edu}
\and
\IEEEauthorblockN{11\textsuperscript{th} Marco A Gerosa}
\IEEEauthorblockA{\textit{SICCS} \\
\textit{Northern Arizona University}\\
Flagstaff, USA \\
marco.gerosa@nau.edu}
}

//ALL TEAMS

// Present the results in one or more tables (TEAM PREDICTIONs)
// Explain the table

// Present the results in one or more pictures (TEAM PREDICTIONs)
// Explain the picture
// Run the stats and show the results (ALL TEAMS)

\section{Discussion}\label{sec:discussion}
// ALL TEAMS
// Let's discuss the findings
// How interesting are they?
// How do they compare with the related work studies
// Is there any other baseline we can compare
// Is there any study (not mention before) that we can mention, given the results

// ALL TEAMS
//Summarize the problem, the results and the main topic discussed. 

// mention future work (possible directions) 
//ALL TEAMs: what will you be doing next in your team?

\section*{Acknowledgment}

// Who is paying the bill?

\begin{table}[htbp]
\centering
\small
\caption{Performance Metrics Ordered by Precision}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
Results                                   & Precision & Recall & F-M*  \\
\hline
%SkillScope RF + TF-IDF & \textbf{0.947} & \textbf{0.981} & \textbf{0.964} \\
%Santos et al. RF+TF-IDF*3\cite{santos2023tell}& \textbf{0.920} & \textbf{0.962} & \textbf{0.940} \\
SkillScope RF + TF-IDF & \textbf{0.908} & \textbf{0.876} & \textbf{0.889} \\

Santos et al. RF+TF-IDF*4 \cite{santos2023tag}& 0.864 & 0.836 & 0.849 \\
Santos et al. RF+TF-IDF\cite{santos2023tell}& 0.842 & 0.835 & 0.838 \\

Vargovich et al. RF+TF-IDF\cite{joe2023give} & 0.806 & 0.782 & 0.793 \\
Vargovich et al. BERT\cite{joe2023give} & 0.791 & 0.606 & 0.686 \\
SkillScope Single LLM** &0.756 &	0.214 &	0.335 \\
Santos et al. RF+TF-IDF\cite{santos2021can}& 0.755 & 0.747 & 0.751 \\
SkillScope*3 Two Tier LLM &0.735 &	0.735 &	0.735 \\
Santos et al. BERT*4 \cite{santos2023tag} & 0.616 & 0.592 & 0.596 \\
%SkillScope LLM & 0.461 &	0.507	& 0.337 \\

\hline
*F-M - F-measure **class = 1 *3 average *4PowerToys project\\
%\\
%*3PowerToys project \\
\end{tabular}
%}

==> rf_performance.tex <==
Average                                   & Precision (1) & Recall (1) & F1 (1)  \\
\hline % \hline
% Big Data                                  & 1.0      & 0.67          & 1.0        & 0.8    & 1.0           & 1.0        & 1.0    \\
% Big Data-Data Processing                  & 1.0      & 0.67          & 1.0        & 0.8    & 1.0           & 1.0        & 1.0    \\
% Test-Unit Testing                         & 1.0      & 0.93          & 1.0        & 0.96   & 1.0           & 1.0        & 1.0    \\
% Input-Output-Data Writing                 & 1.0      & 0.71          & 1.0        & 0.83   & 1.0           & 1.0        & 1.0    \\
% Search-Ranking                            & 1.0      & 1.0           & 0.83       & 0.91   & 1.0           & 1.0        & 1.0    \\
% Natural Language Processing-Text Analysis & 0.99     & 0.91          & 0.91       & 0.91   & 1.0           & 1.0        & 1.0    \\
% Test                                      & 0.99     & 0.92          & 0.92       & 0.92   & 1.0           & 1.0        & 1.0    \\
% Data Structure                            & 0.99     & 0.99          & 1.0        & 0.99   & 1.0           & 0.74       & 0.85   \\
% Security-Authorization                    & 0.99     & 0.94          & 0.8        & 0.86   & 0.99          & 1.0        & 0.99   \\
% Security-Authentication                   & 0.99     & 0.94          & 0.81       & 0.87   & 0.99          & 1.0        & 0.99   \\
% Geographic Information System-Mapping     & 0.99     & 0.71          & 1.0        & 0.83   & 1.0           & 0.99       & 0.99   \\
% Language-Language Extensions              & 0.99     & 0.85          & 0.89       & 0.87   & 1.0           & 0.99       & 0.99   \\
% Software Development and IT Operations    & 0.99     & 0.99          & 1.0        & 0.99   & 1.0           & 0.73       & 0.84   \\
% Utility-Data Conversion                   & 0.99     & 0.92          & 0.85       & 0.88   & 0.99          & 1.0        & 0.99   \\
% Input-Output-Buffering Strategies         & 0.99     & 0.84          & 0.91       & 0.87   & 1.0           & 0.99       & 0.99   \\
% \hline
Micro                              & 0.86          & 0.93   & 0.89       \\
Macro                              & 0.86          & 0.93       & 0.89    \\
\hline
Average & Precision (0) & Recall (0) & F1 (0) \\
Micro & 1.0           & 0.96       & 0.98   \\
Macro & 1.0           & 0.96       & 0.98  \\

%Micro                              & 0.99     & 0.86          & 0.93       & 0.89   & 1.0           & 0.96       & 0.98   \\
%Macro                              & 0.99     & 0.86          & 
%0.93       & 0.89   & 1.0           & 0.96       & 0.98  


